Representing Shape Collections with Alignment-Aware Linear Models

In this paper, we revisit the classical representation of 3D point clouds as linear shape models. Our key insight is to leverage deep learning to represent a collection of shapes as affine transformations of low-dimensional linear shape models. Each linear model is characterized by a shape prototype, a low-dimensional shape basis and two neural networks. The networks take as input a point cloud and predict the coordinates of a shape in the linear basis and the affine transformation which best approximate the input. Both linear models and neural networks are learned end-to-end using a single reconstruction loss. The main advantage of our approach is that, in contrast to many recent deep approaches which learn feature-based complex shape representations, our model is explicit and every operation occurs in 3D space. As a result, our linear shape models can be easily visualized and annotated, and failure cases can be visually understood. While our main goal is to introduce a compact and interpretable representation of shape collections, we show it leads to state of the art results for few-shot segmentation.

==> figures/reconstructions.tex <==
\setsepchar{ }
\readlist\arg{0 5 6 7 9 12 13}
\protorec{SN}{12}{\arg}

\readlist\arg{7 9 13 15 1 9}
\protorec{SN}{22}{\arg}

\readlist\arg{1 4 6 7 8 9}
\protorec{SN}{29}{\arg}

\readlist\arg{0 3 8 7 9 1}
\protorec{SN}{31}{\arg}

\readlist\arg{0 3 6 9 11 13}
\protorec{SN}{33}{\arg}

\readlist\arg{0 1 3 4 5 6}
\protorec{SN}{56}{\arg}

\readlist\arg{0 6 7 9 11 12}
\protorec{SN}{13}{\arg}
